IndicBART: A Pre-trained Model for Indic Natural Language Generation

In this paper, we study pre-trained sequence-to-sequence models for a group of related languages, with a focus on Indic languages. We present IndicBART, a multilingual, sequence-to-sequence pre-trained model focusing on 11 Indic languages and English. IndicBART utilizes the orthographic similarity between Indic scripts to improve transfer learning between similar Indic languages. We evaluate IndicBART on two NLG tasks: Neural Machine Translation (NMT) and extreme summarization. Our experiments on NMT and extreme summarization show that a model specific to related languages like IndicBART is competitive with large pre-trained models like mBART50 despite being significantly smaller. It also performs well on very low-resource translation scenarios where languages are not included in pre-training or fine-tuning. Script sharing, multilingual training, and better utilization of limited model capacity contribute to the good performance of the compact IndicBART model.

==> datasets.tex <==
We describe the Indic NLG datasets we have created or used for our experiments.
\subsection{Existing Datasets}

\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc|c|c}
& \multicolumn{3}{c|}{\textbf{Fine-Tuning}} & \multicolumn{1}{c}{\textbf{Scratch}}\\ \hline
\textbf{Pair} & \textbf{PMI} & \textbf{PIB} & \textbf{Total} & \textbf{Samanantar}\\ \hline
bn-en             & 23,306       & 91,985  & 115,291 &  8,435,620\\
gu-en             & 41,578        & 58,264  & 99,842 &  3,019,563\\
hi-en             & 50,349        & 266,545  & 316,894 &  8,467,772\\
kn-en             & 28,901        & -   & 28,901 &4,014,931\\
ml-en             & 26,916        & 43,087   & 70,003  & 5,780,479\\
mr-en             & 28,974        & 114,220  & 143,194  & 3,288,874\\
or-en             & 31,966        & 94,494   & 126,460 & 990,466\\
pa-en             & 28,294        & 101,092  & 129,386  & 2,400,659\\
ta-en             & 32,638        & 115,968  & 148,606 &  5,095,763\\
te-en             & 33,380 & 44,720 & 78,100&4,775,516\\
\hline
Total             &  326,302      & 930,375 & 1,256,677 & 46,269,643\\

\hline
\end{tabular}}
\caption{Bilingual corpora statistics for the PMI and CVIT-PIB dataset.}
\label{tab:databi}

\end{table}

\subsubsection{Machine Translation}
We benchmark our MT models on the WAT 2021 MultiIndicMT test set and the relevant portion of the FLORES101 devtest \RP{cite these datasets}. We chose these evaluation datasets as it covers all the Indic languages we trained our IndicBART model on, except for Assamese. The WAT2021 development and test sets contain 1,000 and 2,390 11-way sentences. The FLORES devtest set contains 1,012 sentences. As for the training data, we used only the PMI and CVIT-PIB portion for fine-tuning and the Samanantar data for training models from scratch. The PMI and CVIT-PIB data is included in the Samanantar data but domains of the former are quite close to that of the WAT2021 development and test sets. The statistics of these corpora are given in Table~\ref{tab:databi}. The FLORES devtest set is rather challenging as it is distant from the PMI, CVIT-PIB and Samanantar datasets. To make this even more challenging we do not choose any specific fine-tuning data for benchmarking on it. Instead we use the models trained on the aforementioned training data and decode the FLORES devtest set. As we do not use any domain specific fine-tuning data for FLORES, we use the WAT2021 devlopment set to determine the convergence of the models we train. By comparing the performance of models trained from scratch on the general domain Samanantar data and those fine-tuned on the PMI+CVIT-PIB data on two different benchmarking datasets, we should get a clear idea of what to expect in low and high-resource settings in easy and difficult domains when pre-training is used. 

\begin{table}[]
    \centering
    \begin{tabular}{c|ccc}
\textbf{Language} & \textbf{Train} & \textbf{Dev} & \textbf{Test} \\\hline
bn & 8,102 & 1,012 & 1,012 \\
gu & 9,119 & 1,139 & 1,139 \\
hi & 70,778 & 8,847 & 8,847 \\
mr & 10,903 & 1,362 & 1,362 \\
pa & 8,215 & 1,026 & 1,026 \\
ta & 16,222 & 2,027 & 2,027 \\
te & 10,421 & 1,302 & 1,302 \\\hline

    \end{tabular}
    \caption{Statistics of the Indic portion of the multilingual XSum dataset that we used for training our summarization models.}
    \label{tab:xsumdata}
\end{table}

\subsubsection{Summarization}
We used the multilingual XSum dataset \cite{hasan-etal-2021-xl} also known as the XL-Sum dataset. The Indic languages we focus on for evaluating our IndicBART models are: Bengali, Gujarati, Hindi, Marathi, Punjabi, Tamil and Telugu. Additionally, when evaluating mBART25 and mBART50, we consider Sinhala, Nepalese and Urdu. We use the official splits\footnote{\url{https://github.com/csebuetnlp/xl-sum/}} which differ from the splits in \cite{hasan-etal-2021-xl}. The corpora statistics are given in Table~\ref{tab:xsumdata}.


